Random Offset Block Embedding Array (ROBE) for CriteoTB Benchmark MLPerf DLRM Model : 1000$\times$ Compression and 3.1$\times$ Faster Inference

Deep learning for recommendation data is one of the most pervasive and challenging AI workload in recent times. State-of-the-art recommendation models are one of the largest models matching the likes of GPT-3 and Switch Transformer. Challenges in deep learning recommendation models (DLRM) stem from learning dense embeddings for each of the categorical tokens. These embedding tables in industrial scale models can be as large as hundreds of terabytes. Such large models lead to a plethora of engineering challenges, not to mention prohibitive communication overheads, and slower training and inference times. Of these, slower inference time directly impacts user experience. Model compression for DLRM is gaining traction and the community has recently shown impressive compression results. In this paper, we present Random Offset Block Embedding Array (ROBE) as a low memory alternative to embedding tables which provide orders of magnitude reduction in memory usage while maintaining accuracy and boosting execution speed. ROBE is a simple fundamental approach in improving both cache performance and the variance of randomized hashing, which could be of independent interest in itself. We demonstrate that we can successfully train DLRM models with same accuracy while using $1000 \times$ less memory. A $1000\times$ compressed model directly results in faster inference without any engineering effort. In particular, we show that we can train DLRM model using ROBE array of size 100MB on a single GPU to achieve AUC of 0.8025 or higher as required by official MLPerf CriteoTB benchmark DLRM model of 100GB while achieving about $3.1\times$ (209\%) improvement in inference throughput.

==> background.tex <==
\section{Background}
In this section, we introduce a hashing scheme that we will leverage in our implementation of \rmaa.
\subsection{Universal Hashing}


==> figure_main.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.45]{Neurips/rma_scmafigures/auc_evol.png}
    \label{fig:evol}
    \caption{Evolution plots : Original vs UMA}
\end{figure}



==> method.tex <==
\section{Universal Memory Allocation (UMA)}
In UMA, the high-level goal is to use significantly smaller embedding tables, while retaining performance. In other words, we want to virtually use the exact same embedding tables, as required in the model, while using significant smaller amounts of actual memory.
%With UMA, we want to virtually use the exact same embedding tables as required in the model while using a small concrete memory behind the scenes. 
The basic idea is to share weights among the embedding table entries. The approach is inspired from the HashedNet \cite{hashtrick}, where weight sharing is imposed among weight matrices in neural network layers. In UMA, we use a universal hashing function $h \in \mathcal{H}$, where $\mathcal{H}$ is the universal hash family, to map each entry of the embedding tables into a single memory $M$. A sample mapping of elements from 3 embedding tables into a small piece of memory $M$ is shown via color-coding in Figure~\ref{fig:forward}. 

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/UMA-forward.png}
    \caption{Color coding shows the mapping from each of tables into a single memory M. The figure also shows how a typical forward pass lookup of the embedding under UMA looks like.}
    \label{fig:forward}
\end{figure}

\textbf{Forward Pass.}
The forward pass requires looking up the embedding for the given value of a categorical feature. In the original (or full fledged) embedding table, this operation is simply indexing into the embedding matrix at the location of the categorical value, say $x$, and reading the embedding at that location. While in UMA, the lookup of each element is redirected into the memory $M$ using a universal hash function. Under UMA, the embedding for a value $x$ in embedding table $e$ is computed as follows:
\begin{equation*}
    E_{UMA}(x) = (M[h(e, x, 1)], M[h(e, x, 2)], M[h(e, x, 3)], ...,  M[h(e, x, d)]).
\end{equation*}

\textbf{Backward Pass.}
In the backward pass, the gradients of all the elements from the embedding table that map into a single location in $M$ are aggregated into that location. This is illustrated in Figure~\ref{fig:backward}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/UMA-backward.png}
    \caption{ Aggregation of gradients in backward pass }
    \label{fig:backward}
\end{figure}







==> n_method.tex <==
    \begin{table*}[]
    \centering
    \caption{Number of memory fetches on varying sizes of $Z$, where $d$ is the embedding size, $B$ is the bus size and $Z$ is the block size. $B | d$ denotes $B$ divides $d$.}
\begin{tabular}{|l|l|l|l|}
\hline
                          & \textbf{Condition} & \textbf{Max number of memory fetches} & \textbf{Comment}                                          \\ \hline
Original                  & $B | d$              & $d/B + 1$                               &                                                           \\ \hline
\rmaz $Z < B < d$ & $Z | B | d$          & $2 \times d/Z$                               & With high probability as $|M| \gg d >  Z$ \\ \hline
\rmaz $B < Z < d$ & $B | Z | d$          & $d/B + d/Z$                           & With high probability as $|M| \gg d > Z$ \\ \hline
\rmaz $Z \geq d$                & $d | Z$              & $d/B + 2$                             &                                                           \\ \hline
\end{tabular}
\label{tab:memfetches}
\end{table*}
    

\section{\rmafull}
    In the context of models, the memory footprint of the model is determined by the memory used to store the parameters of the model. Generally, each parameter of the model is stored in memory in a separate individual location. However, in the case when the number of parameters far exceed the total amount of memory we intend to use, there are approaches such as pruning or precision-reduction used to fit the parameters in the memory. While these approaches have proven to be useful, the factor of reduction using these approaches is generally quite small. For further reduction in memory footprint of the model, the weights can share memory locations. We achieve this memory sharing via memory allocation functions which we describe below. Once we have a allocation function, say $h$, the forward pass accesses the memory via the allocation function -- if you want to access some parameter $p$, it is accessed at the location $h(p)$. The backward pass aggregates the gradients from all the parameters that share a particular memory location. The memory allocation function along with the associated forward and backward passes are described below. As we will see in Section \ref{sec:theory}, in learning a shared memory, we can expect to get good performing models even with very high compression. This is further supported by our experiments in Section \ref{sec:experiments}.
    
    
    \subsection{\rma-$\pmb{1}$ : {\rma} with block size $\pmb{1}$}
    We begin by describing \rma with a block size of $1$ as it is easier to convey. Subsequently, we will describe \rmaz, which allows for an arbitrary block size of $Z$. 
    
    
    

    
    
    \textbf{Memory Allocation Function:}
    In this paper, we are interested in allocating parameters of embedding tables to a smaller memory, say $M$. We use hash functions to achieve this allocation. We need to ensure that these hash functions are {\em small} to store and {\em fast} to compute. Hence, we use universal hash functions \cite{carter1979universal}, which have $\mathcal{O}(1)$ space usage, $\mathcal{O}(1)$ computation cost, and are convenient to implement over a GPU for parallel computation. Specifically, in our implementation we use,
    \begin{equation}
        h(e, x, i) = (A \times e + B \times x + C \times i + D) \mod P \mod |M|, \label{eq:eq_rma1}
    \end{equation}
    where $e$ is the id of embedding table, $x$ is the token for which we want the embedding, and $i$ is the index inside the embedding. $A, B, C, D,$ and $P$ are standard parameters of universal hashing. This hash function is a light-weight replacement of a random hash function which tries to minimize the collisions among different elements of the embedding table.
    
    In principal, this memory allocation is very similar to Hash-Net \cite{hashtrick}. However, there are differences: (1) we use light-weight universal hashing as opposed to "xxhash" in Hash-Net. Using universal hashing makes implementing the computation on GPU very convenient and efficient (2) Hash-Net keeps separate arrays for separate matrices, whereas we use a single array to map all the elements from all the embedding tables (3) Hash-Net was demonstrated on multi-layered neural networks, and we focus on embedding tables, and (4) most importantly, our view of the memory allocation allows us to extend \rma-$1$ to \rmaz. We show that \rmaz is theoretically superior to \rma-$1$ (described in Section \ref{sec:theory}) and provides coalesced access pattern which improves memory access efficiency by reducing the number of memory fetches. 
    
    \textbf{Forward Pass:} With universal memory allocation function for \rma-$1$, we illustrate the forward pass using Figure\ref{fig:forward}. The forward pass requires looking up the embedding for the given token of a categorical feature. In the original (or full fledged) embedding table, this operation is simply indexing into the embedding matrix at the location of the categorical token, say $x$, and reading the embedding at that location. In \rma-$1$, the lookup of each element is redirected into the memory $M$ using a universal memory allocation function described above. Optionally, each element that is read from the memory is multiplied by a sign $\{+1,-1\}$ which is obtained by another independent universal hash function $g(e,x,i)$.
    
    \textbf{Backward Pass:} With universal memory allocation, the backward pass is illustrated in Figure \ref{fig:backward}. The gradient of a single element in shared memory $M$ can be computed by accumulating gradients from all the elements from embedding table that share this particular location.

    
    \subsection{\rmazbold : {\rma } with arbitrary block size $\pmb{Z}$}
    \rmaz is analogous to \rma-$1$. However, here the basic allocation unit is a block of size $Z$ instead of $1$. We will divide the flattened embedding table into blocks of size $Z$ and each block will be mapped into the memory $M$ at locations pointed out by our memory allocation function. Note that the the memory $M$ is not divided into blocks and hence, there can be overlapping blocks with overlap ranging anywhere from 0 to $Z$ locations.
    
    \textbf{Memory Allocation Function:} As with \rma-$1$, we use universal hash functions to allocate memory in \rmaz. The memory allocation function for \rmaz is
%\begin{align}
        %&\mathcal{C}_{id(i)} = (int) i / Z \\
        %Li: I changed the (int) notation to the following. can change back if not good
%        &\mathcal{C}_{id(i)} = \lfloor i / Z \rceil \\
%        &\mathcal{C}_{\textrm{off}(i)} = i \mod Z \\
%        &h(e, x, i) = ((A \times e + B \times x + C \times \mathcal{C}_{id(i)}  + D) \mod P %\mod (|M|) + \mathcal{C}_{\textrm{off}(i)}) \mod (|M|) \label{eq:eq_rmax}
%\end{align}
    \begin{equation}
    \begin{split}
        h(e, & x, i) =\\
        & \left( ((A \times e  + B \times \mathcal{Z}_{\textrm{id}}(x,i)  + C) \mod P \mod (|M|)) \\
        & + \mathcal{Z}_{\textrm{off}}(x, i)\right) \mod (|M|) \\
        \end{split}\label{eq:eq_rmax}
    \end{equation}
    where $\mathcal{Z}_{id}(x,i)$ is the block number to which the $i^{ith}$ element of x belongs to and $\mathcal{Z}_{\textrm{off}}(x, i)$ is the offset at which $i^{th}$ elmement of $x$ is located inside the block. In our implementation, assuming that $x \in \{0,|S| -1\}$ where $S$ is the set of all values and $d$ is the embedding size, we can compute $\mathcal{Z}_{\textrm{id}}$ and $\mathcal{Z}_{\textrm{off}}$ as follows:
    \begin{equation}
    \begin{split}
        \mathcal{Z}_{\textrm{id}}(x,i) =  \lfloor (xd + i ) / Z\rfloor \\
        \mathcal{Z}_{\textrm{off}}(x,i) =  (xd + i ) \mod Z.
        \end{split}
    \end{equation}
    
    Essentially, the start of the block is mapped randomly into the memory address $(|M|)$ and the block is mapped linearly into the block located at the mapped address. While placing this block, if it exceeds the memory size $|M|$, the latter part of the block is continued from the start of the array. So logically, we use a circular array for memory $M$. The memory allocation is illustrated in Figure \ref{fig:rmax}.
    
    \textbf{Forward and Backward pass:} The forward and backward pass is implemented in similar fashion as for \rma-$1$ except that we use the hash function stated in Equation  (\ref{eq:eq_rmax}) instead of Equation (\ref{eq:eq_rma1}). 
    

    
    \subsection{Advantages of \rmazbold}
    
    \textbf{Memory Latency:}
    The most obvious advantage of using a smaller memory for embedding tables is that it can potentially be stored closer to the processing unit. For example, embedding tables with a  collective size of 100GB, when allocated a memory of 100MB (i.e. $1000\times$ reduction), can be stored on last level cache. The original model, in this case, without any memory sharing has to be stored on RAM, or even worse on disk.
    
    \textbf{Memory Fetches:}
    The number of memory fetches can potentially increase when using a \rmaz allocation scheme. We present the number of memory fetches while using \rmaz and compare it against the memory fetches with using original embedding, which is shown in Table \ref{tab:memfetches}.
    
    Consider the original embedding of size $d$ (generally kept in multiples of bus size). Let the bus size be $B$ (generally 32 or 64) . Thus, in order to fetch a single embedding, we would require a maximum of $(d/B + 1)$ memory fetches. As we can see from Table \ref{tab:memfetches}, as we increase the value of $Z$ the number of memory fetches decrease from the $2d/Z$ to $d/B+2$ when $Z$ is greater than $d$. Also, as we will see in section \ref{sec:theory}, the greater the value of $Z$, the better is dimensionality reduction. So it is advisable to set the value of $Z$ to be $\geq d$
    
    \textbf{Dimensionality Reduction:} As we will see in Section \ref{sec:theory}, \rmaz hashing is better than \rma-$1$ in terms of dimensionality reduction. As the value of $Z$ increases, while the estimate of inner products in projected space is unbiased, the variance decreases until $Z$ reaches $|M|$.
    

    
    
    
    
    

    
    

==> rma_1_figure.tex <==
\begin{figure*}
\begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/UMA-forward.png}
   
    \caption{forward} \label{fig:forward}
\end{subfigure}
    \begin{subfigure}{0.47 \textwidth}
    \centering
    \includegraphics[scale=0.25]{figures/UMA-backward.png}
   
    \caption{backward} \label{fig:backward}
    \end{subfigure}
    \caption{(\textbf{Left}) \rma-1 : Color coding shows the mapping from each of tables into a single memory $M$. The figure also shows how a typical forward pass lookup of the embedding under \rma with block size 1. (\textbf{Right}) Aggregation of gradients in backward pass.}
\end{figure*}
